Common Problems in Delay-Based Congestion Control Algorithms: A Gallery of Solutions

Although delay-based congestion control protocols such as FAST promise to deliver better performance than traditional TCP Reno, they have not yet been widely incorporated to the Internet. Several factors have contributed to their lack of deployment. Probably, the main contributing factor is that they are not able to compete fairly against loss-based congestion control protocols. In fact, the transmission rate in equilibrium of delay-based approaches is always less than their fair share when they share the network with traditional TCP-Reno derivatives, that employ packet losses as their congestion signal. There are also other performance impairments caused by the sensitivity to errors in the measurement of the congestion signal (queuing delay) that reduce the efficiency and the intra-protocol fairness of the algorithms. In this paper we report, analyze and discuss some recent proposals in the literature to improve the dynamic behavior of delay-based congestion control algorithms, and FAST in particular. Coexistence of sources reacting differently to congestion, identifying congestion appearance in the reverse path and the persistent congestion problem are the issues specifically addressed.

==> background.tex <==
\section{FAST-TCP Description}
\label{sec:background}

Thus DCA algorithms are more suitable than Reno variants for long fat pipes
where packet losses are too scarce to properly adjust the rate, and for those
applications negatively affected by sudden changes in the transmission rate.
They work on the assumption that it is possible to gain insight into network
status observing the variations in the RTT. The difference between the RTT and
the propagation delay is directly related to the amount of data in transit,
and, the more data in the network, the nearer it is to become congested. So,
adjusting the window size based on these variations, DCA flows keep an
appropriate transmission rate without causing congestion. In contrast,
TCP-Reno and its variants need to drive the network to congestion to receive
the feedback needed to adjust the window. They keep slowly incrementing the
window size until it reaches a point that buffers overflow and packet losses
occur. This leads sources to abruptly reduce their sending rates and the slow
increment phase begins again, preventing Reno flows to fully enjoy all the
available bandwidth.

Both TCP-Vegas and FAST-TCP employ a similar \emph{modus operandi}, in fact,
FAST-TCP can be treated as an improved (faster) version of the
former~\cite{wei06:_fast_tcp}. Throughout the rest of this paper we will focus
on FAST, although most results can also be applied to Vegas with minor or no
adjustments.

To modulate its transmission rate FAST-TCP employs a congestion window
analogous to the one employed by Reno variants. FAST congestion window can be
characterized, at the flow level, by the following dynamic equation:
\begin{equation}
  \label{eq:dynamic_fast}
  \dot w(t) = \gamma \alpha \left(
    1 - \frac{q(t) x(t)}{\alpha}
    \right),
\end{equation}
where $\gamma$ and $\alpha$ are configuration parameters, $q(t)$ is the
instantaneous queueing delay and $x(t)=\frac{w(t)}{d+q(t)}$ is the
transmission rate, $d$ being the round trip propagation delay. This equation
has the property that the variation on the window size is directly
proportional to the distance from equilibrium, yielding to very \emph{fast}
convergence times.

The above dynamic flow level behavior is implemented at the packet level with
the following rule. Every update interval, defined to be a constant time or
some number of RTTs depending on the precise FAST version, the window size is
updated as
\begin{equation}
  w \longleftarrow \gamma \left( \frac{\hat d w}{\hat r} + \alpha \right) +
  (1-\gamma)w,
  \label{eq:wupdate}
\end{equation}
where $\hat d$ is the current estimation of the round trip propagation delay
and $\hat r=\hat d + \hat q$ is an estimation of the round trip time. The
accurate estimation of $d$ is a bit tricky as it can only be correctly
measured in the absence of cross traffic. In practice $\hat d$ is set to the
minimum round trip time observed during the whole transmission. In the end,
this is only a problem when different FAST flows have different
overestimations. As long as all FAST flows make the same error, the fairness
properties are not affected. Later in this paper, we will study this problem
and provide solutions for it. Eq.~\eqref{eq:wupdate} brings light to the
meaning of $\gamma$. In fact it is just a \emph{smoothing factor} or
\emph{gain} that controls the speed of convergence. Its value its taken from
the semi-open range $(0,1]$, although $\gamma=0.5$ is its more common value.

The equilibrium properties of FAST are well established in the
literature~\cite{wei06:_fast_tcp,jin03:_fast_tcp} and coincide with those of
Vegas~\cite{Low02,samios03:_model_throug_of_tcp_vegas}. In fact,  it is a
direct consequence of its dynamic equation~\eqref{eq:dynamic_fast}. It
suffices to make $\dot w(t)=0$ to obtain that under equilibrium each
connection attains a throughput
\begin{equation}
  \label{eq:fast-tput-equilibrium}
  x^* = \frac{\alpha}{q^*} = \frac{\alpha}{\hat r^* - \hat d}.
\end{equation}
This equilibrium formula merits some observations. Firstly, as long as all
FAST flows share the same configuration (same $\alpha$ value) and bottleneck,
they all obtain the same throughput, irrespectively of their propagation
delays. Secondly, it helps as to get insight in what is the effect of the
$\alpha$ parameter. In fact, if all the flows sharing a bottleneck, and thus
observing the same queueing delay ($\hat r^* - \hat d$), are set up with the
same $\alpha$ parameter, they will get the same equilibrium transmission rate
$x^*_i = x^*$. It soon follows then that
\begin{equation}
  \label{eq:enqueued-packets}
  (\hat r^* - \hat d)\sum_{i=1}^n x_i^* = (\hat r^* - \hat d)C = n\alpha,
\end{equation}
for $n$ flows and link capacity $C$. Finally, solving for $\alpha$
in~\eqref{eq:enqueued-packets} it becomes apparent that each flow contributes
$\alpha$ packets to the bottleneck backlog.

There is a trade off for selecting an appropriate $\alpha$ value. On the one
hand we want to select a small value, to minimize overall latency and buffering
needs in the network. On the other hand, big values provide faster convergence
times. At the same time, too small $\alpha$ values can produce too little
queueing delays making their precise measure too difficult for end hosts.

Lastly, it must also be taken into consideration that not every combination of
$\alpha$ and $\gamma$ produces stable configurations. Several papers deal with
the conditions that both $\alpha$ and $\gamma$ must met to reach equilibrium.
More details can be researched
in~\cite{wang05:_model_and_stabil_of_fast_tcp,choi05:_global_stabil_of_fast_tcp,choi06:_global_expon_stabil_of_fast_tcp,tan07:_param_tunin_for_fast_tcp}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "advances"
%%% End: 

